A charge-preserving method for solving graph neural diffusion networks

The aim of this paper is to give a systematic mathematical interpretation of the diffusion problem on which Graph Neural Networks (GNNs) models are based. The starting point of our approach is a dissipative functional leading to dynamical equations which allows us to study the symmetries of the model. We discuss the conserved charges and provide a charge-preserving numerical method for solving the dynamical equations. In any dynamical system and also in GRAph Neural Diffusion (GRAND), knowing the charge values and their conservation along the evolution flow could provide a way to understand how GNNs and other networks work with their learning capabilities.

==> bibliography.tex <==
\bibitem{higham}Blanchard, P., Higham, D. \& Higham, N. Accurately computing the log-sum-exp and softmax functions. {\em IMA J. Numer. Anal.}. \textbf{41}, 2311-2330 (2021), https://doi.org/10.1093/imanum/draa038
\bibitem{ortiz}Mielke, A. \& Ortiz, M. A class of minimum principles for characterizing the trajectories and the relaxation of dissipative systems. {\em ESAIM Control Optim. Calc. Var.}. \textbf{14}, 494-516 (2008), https://doi.org/10.1051/cocv:2007064
\bibitem{hairer}Hairer, E., Lubich, C. \& Wanner, G. Geometric numerical integration. (Springer-Verlag, Berlin,2006), Structure-preserving algorithms for ordinary differential equations
\bibitem{gradient-flow}Mielke, A. \& Stefanelli, U. Weighted energy-dissipation functionals for gradient flows. {\em ESAIM Control Optim. Calc. Var.}. \textbf{17}, 52-85 (2011), https://doi.org/10.1051/cocv/2009043
\bibitem{evans2022partial}Evans, L. Partial differential equations. (American Mathematical Society,2022)
\bibitem{MB}Bronstein, M., Bruna, J., LeCun, Y., Szlam, A. \& Vandergheynst, P. Geometric Deep Learning: Going beyond Euclidean data. {\em IEEE Signal Processing Magazine}. \textbf{34} pp. 18-42 (2016)
\bibitem{GRAND}Chamberlain, B., Rowbottom, J., Gorinova, M., Webb, S., Rossi, E. \& Bronstein, M. GRAND: Graph Neural Diffusion. {\em International Conference On Machine Learning}. (2021)
\bibitem{GREAND}Choi, J., Hong, S., Park, N. \& Cho, S. GREAD: Graph Neural Reaction-Diffusion Equations. {\em CoRR}. \textbf{abs/2211.14208} (2022), https://doi.org/10.48550/arXiv.2211.14208
\bibitem{chamberlain2021beltrami}Chamberlain, B., Rowbottom, J., Eynard, D., Giovanni, F., Dong, X. \& Bronstein, M. Beltrami Flow and Neural Diffusion on Graphs.  (2021)
\bibitem{gilmore}Gilmore, R. Lie groups, Lie algebras, and some of their applications. (Robert E. Krieger Publishing Co., Inc., Malabar, FL,1994), Reprint of the 1974 original
\bibitem{GAT}Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A., Kaiser, Ł. \& Polosukhin, I. Attention is all you need. {\em Advances In Neural Information Processing Systems}. \textbf{30} (2017)
\bibitem{Bronstein_2017}Bronstein, M., Bruna, J., LeCun, Y., Szlam, A. \& Vandergheynst, P. Geometric Deep Learning: Going beyond Euclidean data. {\em IEEE Signal Processing Magazine}. \textbf{34}, 18-42 (2017,7), http://dx.doi.org/10.1109/MSP.2017.2693418
\bibitem{digiovanni2023understanding}Giovanni, F., Rowbottom, J., Chamberlain, B., Markovich, T. \& Bronstein, M. Understanding convolution on graphs via energies.  (2023)
\bibitem{cheng2023graph}Cheng, H., Zhou, J., Tay, W. \& Wen, B. Graph Neural Networks With Triple Attention for Few-Shot Learning. {\em IEEE Transactions On Multimedia}. (2023)
\bibitem{di2022graph}Di Giovanni, F., Rowbottom, J., Chamberlain, B., Markovich, T. \& Bronstein, M. Graph neural networks as gradient flows. {\em ArXiv Preprint ArXiv:2206.10991}. (2022)
\bibitem{digiovanni2022heterogeneous}Giovanni, F., Luise, G. \& Bronstein, M. Heterogeneous manifolds for curvature-aware graph embedding.  (2022)
\bibitem{lutter2019deep}Lutter, M., Ritter, C. \& Peters, J. Deep Lagrangian Networks: Using Physics as Model Prior for Deep Learning.  (2019)
\bibitem{cranmer2020lagrangian}Cranmer, M., Greydanus, S., Hoyer, S., Battaglia, P., Spergel, D. \& Ho, S. Lagrangian Neural Networks.  (2020)
\bibitem{greydanus2019hamiltonian}Greydanus, S., Dzamba, M. \& Yosinski, J. Hamiltonian neural networks. {\em Advances In Neural Information Processing Systems}. \textbf{32} (2019)
\bibitem{liu2021machine}Liu, Z. \& Tegmark, M. Machine learning conservation laws from trajectories. {\em Physical Review Letters}. \textbf{126}, 180604 (2021)
\bibitem{liu2022machine}Liu, Z., Madhavan, V. \& Tegmark, M. Machine learning conservation laws from differential equations. {\em Physical Review E}. \textbf{106}, 045307 (2022)
\bibitem{mattheakis2020physical}Mattheakis, M., Protopapas, P., Sondak, D., Giovanni, M. \& Kaxiras, E. Physical Symmetries Embedded in Neural Networks.  (2020)
\bibitem{bondesan2019learning}Bondesan, R. \& Lamacraft, A. Learning Symmetries of Classical Integrable Systems.  (2019)
\bibitem{wang2023scientific}Wang, H., Fu, T., Du, Y., Gao, W., Huang, K., Liu, Z., Chandak, P., Liu, S., Van Katwyk, P., Deac, A. \& Others Scientific discovery in the age of artificial intelligence. {\em Nature}. \textbf{620}, 47-60 (2023)
\bibitem{forestano2023deep}Forestano, R., Matchev, K., Matcheva, K., Roman, A., Unlu, E. \& Verner, S. Deep learning symmetries and their Lie groups, algebras, and subalgebras from first principles. {\em Machine Learning: Science And Technology}. (2023)
\bibitem{hagemeyer2022learning}Hagemeyer, C. Learning Linear Symmetries in Data Using Moment Matching.  (2022)

